Searching a Database of Source Codes Using Contextualized Code Search

Consider the case where a programmer has written some part of a program, but has left part of the program (such as a method or a function body) incomplete. The goal is to use the context surrounding the missing code to automatically 'figure out' which of the codes in the database would be useful to the programmer in order to help complete the missing code. The search is 'contextualized' in the sense that the search engine should use clues in the partially-completed code to figure out which database code is most useful. The user should not be required to formulate an explicit query. We cast contextualized code search as a learning problem, where the goal is to learn a distribution function computing the likelihood that each database code completes the program, and propose a neural model for predicting which database code is likely to be most useful. Because it will be prohibitively expensive to apply a neural model to each code in a database of millions or billions of codes at search time, one of our key technical concerns is ensuring a speedy search. We address this by learning a 'reverse encoder' that can be used to reduce the problem of evaluating each database code to computing a convolution of two normal distributions.

==> Application/GuiAppl/qry_0.tex <==
import javax.swing.*;

class MyGuiAppl{

    /**
    create a new frame
    */
    public JFrame <?>(<?> a){
        __CODE_SEARCH__();
    }
}




==> Application/GuiAppl/qry_0_rank6.tex <==
 /** 
  * Creates a new UserInterface object.
  * @param title the title
  * @return the j frame
  */
 public JFrame createFrame(final String title){
   JFrame frame=new JFrame(title);
   return frame;
 }


==> Application/GuiAppl/qry_1.tex <==
    .
    .
    /**
    create button
    */
    public <?> <?>(<?> a){
        __CODE_SEARCH__();
    }
}


==> Application/GuiAppl/qry_1_rank7.tex <==
 private JButton makeButton(String arg){
   JButton button=new JButton(arg);
   return button;
 }


==> Application/GuiAppl/qry_2.tex <==
    .
    .
    
    public void actionClose(
                 JButton a, JFrame f){
        __CODE_SEARCH__(); 
    }
}



==> Application/GuiAppl/qry_2_rank0.tex <==
 private void setCloseSurrogateButtonAction
          (JButton closeSurrogateButton,JFrame guiFrame){
   closeSurrogateButton.addActionListener
                                    (new ActionListener(){
     public void actionPerformed( ActionEvent event){
       closeString=CLOSE_UI_EXIT_SURROGATE;
       guiFrame.dispatchEvent(new WindowEvent
                          (guiFrame,WindowEvent.WINDOW_CLOSING));
       if (closingWindow) { surrogate.userExit=true; }
  else {closeString=CLOSE_UI_SURROGATE_KEEPS_RUNNING;}
     }
   }
  );}


==> Experiment/visualize/ASTs/qry_0.tex <==
ArrayList<String>.ArrayList<String>
FileReader.FileReader(String)
BufferedReader.BufferedReader
                 (FileReader)
while
  BufferedReader.readLine ()
do
  String.split(String)
  ArrayList<String>.add(String)


==> Experiment/visualize/ASTs/qry_1.tex <==
FileWriter.FileWriter(String)
BufferedWriter.BufferedWriter
                 (Writer)
Writer.write(String)

==> Experiment/visualize/ASTs/qry_2.tex <==
while
  Iterator<String>.hasNext()
do
  Iterator<String>.next()
  Iterator<String>.remove()


==> Introduction/examples/program0.tex <==
/**
 * Writes the complete contents of this byte 
    array output stream to the specified 
    output stream argument.
 * @param out the output stream to which 
   to write the data.
 * @throws IOException if I/O error occurs.
 */
public void writeTo(OutputStream out) 
                 throws IOException {
  ByteString[] cachedFlushBuffers;
  byte[] cachedBuffer;
  int cachedBufferPos;
synchronized (this) {
    cachedFlushBuffers=flushedBuffers.toArray(
   new ByteString[flushedBuffers.size()]);
    cachedBuffer=buffer;
    cachedBufferPos=bufferPos;
  }
  for(ByteString byteString:cachedFlushBuffers){
    byteString.writeTo(out);
  }
  out.write(copyArray(
      cachedBuffer,cachedBufferPos));
}


==> Introduction/examples/query.tex <==
class IO {
  public void readFully(InputStream fd, 
           byte[] dst, int off, int len) 
                    throws IOException {
      while (len > 0) {
         int r = fd.read(dst, off, len);
         off += r;
         len -= r;
      }
  }
 
  public void missingCode(OutputStream out){
       __CODE_SEARCH__();
  }
}


==> Learning/Learning.tex <==

We begin by describing the learning problem that underlies contextualized code search.  





==> Model/Search.tex <==





==> QueryMatching/query.tex <==
%In this section we briefly talk about the Context Sensitive Search System. There are 3 major components to our system.\\

Finding relevant answers to a query from a database has been long studied in multiple communities including Information Retrieval and Databases. Program search to an user query $x$ reduces to a traditional top-K search from a database whose contents are a set of Programs $Prog$, with their decompiled representations $Y$. Traditionally this problem has been solved by keyword-matching techniques, where $q$ is decomposed into a long list of corresponding keywords and similarity with a program is determined by a function $f$, which measures the contribution of that keyword in the program, if it exists.

The popularity of Neural Network in recent years has also changed the notion of database search. Modern systems try to find representations of both the query $x$ and program $Y$ such that their relative similarity can be mathematically measured.  This makes it possible to reduce such similarity during `training' time and querying for the most similar item durind test. Mathematically the pipeline of search can be best described as a two step process. The learning problem reduces to evaluating a certain model $M$, parametrized by $\theta$, such that it can minimize a certain similarity metric $f$ between queries and programs. Testing, on the other hand, reduces to finding the optimal $P$ for input query $x_{in}$ assuming the model $M$, with its corresponding $\theta^*$, has already been properly trained.


\begin{equation}\label{simple_training}
\begin{aligned}
&\theta^* = \argmax_\theta \sum_{(y,x) \in (Y,X)}f( y, x | \theta ) \\
&prog^* = \argmax_{p, (y,p) \in (Y,Prog)} f( y , x_{in} | \theta^*) 
\end{aligned}
\end{equation}




Mapping two abstract data structures into the same space is a hard problem. Most of the recent works that use Deep Learning for search, would use Neural Networks to learn the low-level features of its components and use that to project them in a shared multi-dimensional space, with the similarity module of choice being cosine distance. In other words, each program is now represented as $d$-dimensional vector of floating points. However these methods suffer from an inherent problem of negative sampling. To avoid the model to converge to a trivial solution where every program gets mapped to the same vector, a standard technique is to use negative sampling. The $(x,y)$ tuple of programs and query is changed to a $(y,x^+,x^-)$ triplet combination and the model is trained to minimize the similarity between $(y,x^+)$ while simultaneously maximizing the similarity between $(y,x^-)$.

%Fundamentally this approach is flawed for context based code search as the possibility of programs sharing components from evidence is high, even though they might be representing completely different functionalities.

For a context based program search problem, defining a negative sample becomes an extremely hard problem. Two programs with entirely different data types and API calls might be co-used fairly often. This results in poor declaration of loss function which subsequently hampers the quality of model trained. We propose a system that can fundamentally learn how to `program'.  We take inspiration from the field of `program synthesis' and keep it as integral part of the training pipeline. In a Bayesian setting, we let program $Y$ be represented as a probabilistic function  of the query $X$, parametrized by a Neural Network. In this setting, training changes to maximizing the log-likelihood of the programs given the queries and search reduces to finding the $Y$ that maximizes the posterior distribution $P(Y|X)$.


\begin{equation}\label{simple_training_bayesian}
\begin{aligned}
&\theta^* = \argmax_\theta \sum_{X,Y}P(Y | X; \theta) \\
&prog^* = \argmax_{p; (y,p) \in (Y,Prog)} P(Y | X; \theta^*)
\end{aligned}
\end{equation}


A practical hindrance to applicability of this approach is query execution time, as a search solution needs to find appropriate solutions in a reasonable amount of time. Parsing an RNN like NN for each program would then be a huge computational task during search. To reduce the program complexity of search, we use Bayes Rule to find a fast approximation of $P(Y|X)$ which reduces to a convolution between learned representations of both the Encoder and Reverse Encoder in a shared latent space $Z$, representing the query representation $P(Z|X)$ and program representation as $Q(Z|Y)$. This results in training a network to maximizing log-likelihood while also learning the proxy distribution of 
$Q(Z|Y)$ and search results in finding programs with the highest posterior values by a mathematical function of simple matrix-vector operations. Note the similarity of search to the cosine-similarity counter-part, which guarantees a fast search, but does not involve any negative sampling which adversely affects the training pipeline. Search finds the $Y$ that maximizes the posterior distribution $P(Y|X)$ which is approximate computed by $g$.

\begin{equation}\label{complex_training_bayesian}
\begin{aligned}
& \theta^* = \argmax_\theta \sum_{X,Y}[P(Y | X; \theta) + KL(Q(Z|Y) || P(Z|Y);\theta)]\\
& prog^* = \argmax_{p; (y,p) \in (Y,Prog)} g(P(Z | X; \theta^*) , P(Z | X; \theta^*)) 
\end{aligned}
\end{equation}



The details of training and search steps are given in section \ref{training} and \ref{search}.

%
%\noindent \textbf{A fast search}: 
%
%Parsing an RNN like NN for each program would then be a huge computational task. To reduce the program complexity of search, we 
%we incorporate a \textit{Reverse Encoder} that maps back from the program space to the latent space $Z$ thereby including $P(Z|Y)$. With this extra distribution in hand, we can. Our final search equation evaluates to:
%
%\begin{equation}
%\begin{aligned}
%D_X = \sum_{d=1}^D f^d(X) + f^d(Y) - f^d(X-Y)  
%\end{aligned}
%\end{equation}
%where $ f = <\frac{B_{1i}^2}{4A_{1i}} + \frac{1}{2}ln(-\frac{A_{2i}}{\pi})$ \\
%
%Indexing programs happens separately and stored them in a database, each of them represented as a vector of floats. Any new program of the same type can also be included without the need for any re-training. The search procedure involves a single pass over all the programs which can be easily parallelized over multiple cores at the disposal of the database server.
%
%\noindent \textbf{Training a NN}: Assume a training corpus of the form $D_t = \{ (\sX_1, \sProg_1),$ $(\sX_2, \sProg_2), ... \}$.  Each $\sProg_i$ is a code fragment from a universe $\mathbb{P}$ (in this paper  we assume that the code fragment is a Java method body), and each $\sX_i$is a set of evidences from a universe $\mathbb{X}$.  A set of evidences 
%describes the programmatic context in which the fragment $\sProg_i$ is found.  
%Typically, $D_t$ is constructed by analyzing a large corpus of programs (such as a set of projects
%downloaded from GitHub \cite{}) and collecting code fragments as well as the evidence surrounding
%each code fragment. We assume this extraction process is embodied by a generative model $F$, 
%where $(\sX_i, \sProg_i) \sim F(\sX_i, \sProg_i)$. Moreover each program is de-normalized to a canonical representation $Y$ using Eclipse Java DOM Driver to yield its corresponding AST. 
%
%There are two major components to our model amenable to training, a \textit{Forward} model consisting of Encoder and Decoder that helps with program synthesis to approximate $P(\sY|\sX, \theta) \approx \int_{\mathbb{P}_{\sY}} F(\sProg | \sX) d\sProg$.  The \textit{Backward} model works to learn a proxy distribution $Q$ that can closely approximate $P(Z|Y)$ by lowering the KL divergence between the two distributions.
%
%
%Then, given a distribution family $P(Y|\sX, \theta)$, the goal when learning to perform contextualized code search is to 
%use $D_t$ to choose $\theta$ so that for any program $\sY$, we maximize $F$ while also simultaneously lowering $KL(Q(Z|Y) || P(Z|Y))$. That is, we seek to use $D_t$ to learn a distribution that approximates $F$, modulo the fact that we do not 
%wish to distinguish between code fragments that decompile into the same sketch.
%
%In effect we maximize a closed form lower-bound derived in section ? that evaluates to
%\begin{equation}\label{eqlearning}
%\begin{aligned}
%\M^*&=\argmax_\M \sum_i \log P(\Sy_i | \Sx_i, \M) - D_{KL}(P(Z|X)\|P(Z))  \\
%& - D_{KL}(Q(Z|Y)\|P(Z|X)) - D_{KL}(P(Z|X)\|Q(Z|Y)) 
%\end{aligned}
%\end{equation}


%


==> RelatedWork/pythia.tex <==
 { \color{red} 
 
 The idea of using deep neural models for code completion in IDEs have also been popular recently, like Pythia \cite{pythia}. From an application point of view, Pythia shares commonalitites with our system, in integrating a modern Deep Learning based engine to assist developer in code development process. Pythia shares the same concerns as ours in terms of model deployment and latency requirements from a systems point of view. Pythia helps an end user by recommending the next API Call by using context from the current partially constructed program.  In constrast, we search for the most similar program method to an incomplete programmer method in an OOP environment using all parts of the program class as well as the method internals. Whereas Pythia solves the API recommendation problem with a sequential Neural Network model for classification, we solve the problem of similar program search using a probabilistic graphical model.  Both of these ideas can be useful to a programmer during development in an IDE. While Pythia can help programmer with recommending the next API Call while writing a method, \textsc{Codec} can lookup for similar programs from a database whenever the user would like to tally his current code with programs already available. 
 

}

==> System/example/program.tex <==
public class TestIO {

  void write(File f){
     ...
  }

  void skip(File f){
     ...
  }

  void read(File file) {
    FileReader fr1;
    BufferedReader br1;
    fr1 = new FileReader(file);
    br1 = new BufferedReader(fr1);
    while ((br1.readLine()) != null) {}
    return;
   }
}



==> Types_of_evidence/Types_of_evidence_extracted.tex <==
\label{sec-evidence}

Our current implementation focuses on contextualized code search for a missing method.
The searches three types of evidence from the program that surrounds the method containing
the missing code fragement: 

(1) \emph{Class Name}; name of the class split using camel-case formating; 
each is encoded with a one layer GRU-RNN network.
(2) \emph{Class types}; types of the instance variables in the same class as the query method; 
each is encoded with a one layer fully-connected network.
(3) \emph{Surrounding Methods}; Methods within the same class; represented as a two-layer fully connected network made up of concatenated values of its components.

(a) \emph{Return types}; return type of methods appearing in the same class; encoded with a one-layer network.
(b) \emph{Input parameter lists}; sequences of (formal parameters, variable names) appearing in method headers within the same class; This is encoded using a nested GRU-RNN, where the variable names are split using camel-case as its sequence of input. The output is concatenated with each formal parameter and serves as input to another GRU-RNN.
(c) \emph{Method Name}; name of the method split using camel-case formating; each is encoded with a one layer GRU-RNN network.
(d) \emph{API call sequences}; API call sequences are extracted from methods within the same class; encoded with a one layer GRU-RNN network.

We also use four types of evidence from the header of the missing method (if available): (1) \emph{JavaDoc};
English text of JavaDoc associated with the method, lemmatized and stop words removed.  Encoded using a  
bidirectional GRU-RNN.  We also use (2) \emph{Method Name}, (3) \emph{Return types} and (4) \emph{Formal parameter lists}, as above.

Finally, we use four types of evidence from within the (partial) code that is being searched for. These may be available if a fragment of the code has already been written. They are: (1) \emph{API calls}; these are the calls in the code; each is encoded with a one-layer network. 
(2) \emph{API call sequences}; these are extracted via symbolic execution of the code; each is encoded using a GRU-RNN.
(3) \emph{Types}; these are the API types in the code; each is encoded with a one-layer network. 
(4) \emph{Keywords}; English-like words extracted from fully qualified name of the classes inside the method body, combined with english words appearing in types and API calls; each is encoded with a one-layer network.



